Scene Graph Modification Based on Natural Language Commands

Structured representations like graphs and parse trees play a crucial role in many Natural Language Processing systems. In recent years, the advancements in multi-turn user interfaces necessitate the need for controlling and updating these structured representations given new sources of information. Although there have been many efforts focusing on improving the performance of the parsers that map text to graphs or parse trees, very few have explored the problem of directly manipulating these representations. In this paper, we explore the novel problem of graph modification, where the systems need to learn how to update an existing scene graph given a new user's command. Our novel models based on graph-based sparse transformer and cross attention information fusion outperform previous systems adapted from the machine translation and graph generation literature. We further contribute our large graph modification datasets to the research community to encourage future research for this new problem.

==> tab_analysis.tex <==
\begin{table}[h]
\begin{center}
{\small
\begin{tabularx}{\linewidth}{p{0.45\linewidth}|p{0.45\linewidth}}\hline
\textbf{src graph} & \textbf{src graph}\\
young man wearing hat & light reflection\\
\textbf{modification query} &\textbf{modification query} \\
Take away his hat .  &I want to see the reflection on the roof in the image .\\
\textbf{reference} & \textbf{reference}\\
young man & light reflection on roof\\
\textbf{cross-attention} & \textbf{cross-attention}\\
young man & light reflection on roof\\
\textbf{GraphTrans.} & \textbf{GraphTrans.}\\
young man hat & reflection on roof\\
\hline
% \textbf{src graph}\\
% light reflection\\
% \textbf{modification query}\\
% I want to see the reflection on the roof in the image . \\
% \textbf{reference}\\
% light reflection on roof\\
% \textbf{cross-attention}\\
% light reflection on roof\\
% \textbf{graphRNN}\\
% reflection on roof\\
% \hline
\end{tabularx}
}
\end{center}
\caption{\label{tb:eg} Our best model vs the Graph Transformer. Graphs are flattened for easier comparison.}
\vspace{-5mm}
\end{table}
%
% \setlength\tabcolsep{1.5pt} % default value: 6pt
% \begin{wraptable}{r}{83mm}
% \vspace{-9mm}
% %\begin{table}[t]
% \begin{center}
% {\small
% \begin{tabularx}{\linewidth}{l||X|X}\toprule
% \textbf{src graph} & yellow shirt & light reflection\\
% \midrule
% {Query} & I want the shirt to be blue instead of yellow & I want to see the reflection on the roof in the image\\
% \hline
% {Ground Truth}& blue shirt & light reflection on roof\\
% \hline
% {Best Config} & blue shirt & light reflection on roof\\
% \hline
% {Base Config} & yellow shirt & reflection on roof\\
% \bottomrule
% \end{tabularx}
% }
% \end{center}
% \caption{Examples of the best vs base configurations of our model. Graphs are flatten for easier comparison.}
% \label{tb:eg} 
% %\end{table}
% \vspace{-3mm}
% \end{wraptable}


==> tab_example.tex <==
\begin{table}[h]
    \centering
    \small{
    \begin{tabular}{l}
    \toprule
         Src:
         men\\
         Query:
         Show me the men with the jackets .\\
         Tgt:
         men \textcolor{red}{with the jackets}\\
        \midrule
         Src:
         door\\
         Query:
         Show me the sliding door instead .\\
         Tgt:
         \textcolor{red}{sliding} door
         \\
         \midrule
         Src:
    young man \textcolor{red}{wearing hat}\\
Query:
Take away his hat\\
Tgt:
young man\\
\midrule
Src:
man \textcolor{red}{playing tennis}\\
Query:
i just need a man\\
Tgt:
man\\
\midrule
Src:
small clock\\
Query:
Show more clocks\\
Tgt:
small \textcolor{red}{clocks}\\
\midrule
Src:
white surfboard \\
Query:
i want a pink surfboard ; it ca n't be white .\\
Tgt:
\textcolor{red}{pink} surfboard\\
        \bottomrule
    \end{tabular}
        }
    \caption{Examples from user-generated dataset. We flatten source and target graphs for the sake of the readability. Changes are highlighted with \textcolor{red}{red} color.}
    \label{tab:examples}
\end{table}

==> tab_graph.tex <==
\begin{table}[h!]
    \centering
    \begin{tabular}{l|c||c|c}
    
     &\multicolumn{3}{c}{Accuracy}\\
    \cline{2-4}
           & Synthetic & Real  & Mix\\
              \hline\hline
     \qquad graphRNN & 74.68   & 53.98 & 61.02\\
     \qquad flat edge & 76.13  &54.70 & 62.13\\
     \qquad gating & 77.04   &  56.00  & 64.87\\
     \qquad cross-attn & 82.97 &   56.37  &67.10\\
     \hline
    \end{tabular}
    \caption{Graph-level matching over synthetic, real and mixture data.}
    \label{tab:graph-acc}
\end{table}

==> tab_realdata.tex <==
% \begin{table*}[h!]
%     \centering
%     \begin{tabular}{l|c|c|c|c||c|c|c|c}
    
%     \multirow{3}{*}{} &\multicolumn{4}{c||}{Edge-level} &\multicolumn{4}{c}{Node-level}\\
%     \cline{2-9}
%     & \multicolumn{2}{c|}{Real} &\multicolumn{2}{c||}{Mix} & \multicolumn{2}{c|}{Real} &\multicolumn{2}{c}{Mix} \\
%      \cline{2-9}
%           & Precision & Recall  & Precision & Recall & Precision & Recall  & Precision & Recall\\
%               \hline\hline
%      \qquad copy src &31.52& 31.33 & - & -&  66.29  &66.06 &- &-\\
%      \qquad graphRNN & 56.80& 52.89 & 62.96 & 59.27& 81.32& 78.42 & 85.46 & 83.21\\
%      \qquad flat edge & 57.30 & 53.37 &63.74 & 60.18 & 81.63 & 78.85 & 85.78&83.32\\
%      \qquad gating & 58.30  & 53.44 & 64.97 & 62.60 &  81.45  & 78.01 &86.55 &84.95 \\
%      \qquad cross-attn & 59.47 & 55.95 &68.56 &  64.76& 82.51  &80.06 &88.60 &86.10\\
%      \hline
%     \end{tabular}
%     \caption{Node-level and edge-level matching over both real and mixture data.}
%     \label{tab:realdata}
% \end{table*}
\begin{table}[h!]
    \centering
    \begin{tabular}{l|c|c||c}
    
    \multirow{2}{*}{} &  \multicolumn{2}{c||}{F1} & Acc. \\
    \cline{2-4}
    & Edge & Node & Graph
   \\
              \hline\hline
     \qquad copy src &31.42 & 66.17 & -\\
     \qquad graphRNN & 54.78 & 79.84  & 53.98\\
     \qquad flat edge & 55.27 & 80.22 &54.70\\
     \qquad gating &55.76  & 79.69  &  56.00\\
     \qquad cross-attn & 57.66 & 81.27&  56.37\\
     \hline
    \end{tabular}
    \caption{Node-level, edge-level and graph-level matching over real data.}
    \label{tab:realdata}
\end{table}
